Calibration of the Logarithmic-Periodic Dipole Antenna (LPDA) Radio Stations at the Pierre Auger Observatory using an Octocopter

An in-situ calibration of a logarithmic periodic dipole antenna with a frequency coverage of 30 MHz to 80 MHz is performed. Such antennas are part of a radio station system used for detection of cosmic ray induced air showers at the Engineering Radio Array of the Pierre Auger Observatory, the so-called Auger Engineering Radio Array (AERA). The directional and frequency characteristics of the broadband antenna are investigated using a remotely piloted aircraft (RPA) carrying a small transmitting antenna. The antenna sensitivity is described by the vector effective length relating the measured voltage with the electric-field components perpendicular to the incoming signal direction. The horizontal and meridional components are determined with an overall uncertainty of 7.4^{+0.9}_{-0.3} % and 10.3^{+2.8}_{-1.7} % respectively. The measurement is used to correct a simulated response of the frequency and directional response of the antenna. In addition, the influence of the ground conductivity and permittivity on the antenna response is simulated. Both have a negligible influence given the ground conditions measured at the detector site. The overall uncertainties of the vector effective length components result in an uncertainty of 8.8^{+2.1}_{-1.3} % in the square root of the energy fluence for incoming signal directions with zenith angles smaller than 60{\deg}.

==> AuthorList/jinstpub_authorlist.tex <==
% created on 2017-02-02

\author[63]{A.~Aab,}
\author[70]{P.~Abreu,}
\author[48,47]{M.~Aglietta,}
\author[29]{I.~Al Samarai,}
\author[16]{I.F.M.~Albuquerque,}
\author[1]{I.~Allekotte,}
\author[8,11]{A.~Almela,}
\author[62]{J.~Alvarez Castillo,}
\author[78]{J.~Alvarez-Mu\~niz,}
\author[38]{G.A.~Anastasi,}
\author[81]{L.~Anchordoqui,}
\author[8]{B.~Andrada,}
\author[70]{S.~Andringa,}
\author[45]{C.~Aramo,}
\author[76]{F.~Arqueros,}
\author[72]{N.~Arsene,}
\author[1,24]{H.~Asorey,}
\author[70]{P.~Assis,}
\author[29]{J.~Aublin,}
\author[9,10]{G.~Avila,}
\author[73]{A.M.~Badescu,}
\author[71]{A.~Balaceanu,}
\author[54]{F.~Barbato,}
\author[70]{R.J.~Barreira Luz,}
\author[86]{J.J.~Beatty,}
\author[31]{K.H.~Becker,}
\author[12]{J.A.~Bellido,}
\author[30]{C.~Berat,}
\author[56,47]{M.E.~Bertaina,}
\author[1]{X.~Bertou,}
\author[b]{P.L.~Biermann,}
\author[29]{P.~Billoir,}
\author[28]{J.~Biteau,}
\author[12]{S.G.~Blaess,}
\author[70]{A.~Blanco,}
\author[25]{J.~Blazek,}
\author[50,43]{C.~Bleve,}
\author[25]{M.~Boh\'a\v{c}ov\'a,}
\author[40,d]{D.~Boncioli,}
\author[22]{C.~Bonifazi,}
\author[67]{N.~Borodai,}
\author[8,33]{A.M.~Botti,}
\author[h]{J.~Brack,}
\author[71]{I.~Brancus,}
\author[35]{T.~Bretz,}
\author[33]{A.~Bridgeman,}
\author[35]{F.L.~Briechle,}
\author[37]{P.~Buchholz,}
\author[77]{A.~Bueno,}
\author[63]{S.~Buitink,}
\author[52,42]{M.~Buscemi,}
\author[60]{K.S.~Caballero-Mora,}
\author[53]{L.~Caccianiga,}
\author[11,8]{A.~Cancio,}
\author[63]{F.~Canfora,}
\author[72]{L.~Caramete,}
\author[52,42]{R.~Caruso,}
\author[48,47]{A.~Castellina,}
\author[43]{G.~Cataldi,}
\author[70]{L.~Cazon,}
\author[61]{A.G.~Chavez,}
\author[17]{J.A.~Chinellato,}
\author[25]{J.~Chudoba,}
\author[12]{R.W.~Clay,}
\author[8]{A.~Cobos,}
\author[54,45]{R.~Colalillo,}
\author[87]{A.~Coleman,}
\author[47]{L.~Collica,}
\author[50,43]{M.R.~Coluccia,}
\author[70]{R.~Concei\c{c}\~ao,}
\author[53]{G.~Consolati,}
\author[9,10]{F.~Contreras,}
\author[12]{M.J.~Cooper,}
\author[87]{S.~Coutu,}
\author[79]{C.E.~Covault,}
\author[88]{J.~Cronin,}
\author[49,43]{S.~D'Amico,}
\author[17]{B.~Daniel,}
\author[5,3]{S.~Dasso,}
\author[33]{K.~Daumiller,}
\author[12]{B.R.~Dawson,}
\author[23]{R.M.~de Almeida,}
\author[63,65]{S.J.~de Jong,}
\author[63]{G.~De Mauro,}
\author[22]{J.R.T.~de Mello Neto,}
\author[50,43]{I.~De Mitri,}
\author[23]{J.~de Oliveira,}
\author[15]{V.~de Souza,}
\author[33]{J.~Debatin,}
\author[28]{O.~Deligny,}
\author[55,46]{C.~Di Giulio,}
\author[51,41]{A.~Di Matteo,}
\author[17]{M.L.~D\'\i{}az Castro,}
\author[70]{F.~Diogo,}
\author[17]{C.~Dobrigkeit,}
\author[62]{J.C.~D'Olivo,}
\author[37]{Q.~Dorosti,}
\author[21]{R.C.~dos Anjos,}
\author[4]{M.T.~Dova,}
\author[36]{A.~Dundovic,}
\author[25]{J.~Ebr,}
\author[33]{R.~Engel,}
\author[35]{M.~Erdmann,}
\author[37]{M.~Erfani,}
\author[f]{C.O.~Escobar,}
\author[70]{J.~Espadanal,}
\author[8,11]{A.~Etchegoyen,}
\author[63,66,65]{H.~Falcke,}
\author[84]{G.~Farrar,}
\author[17]{A.C.~Fauth,}
\author[f]{N.~Fazzini,}
\author[56]{F.~Fenu,}
\author[83]{B.~Fick,}
\author[8]{J.M.~Figueira,}
\author[74,75]{A.~Filip\v{c}i\v{c},}
\author[73]{O.~Fratu,}
\author[6]{M.M.~Freire,}
\author[88]{T.~Fujii,}
\author[8,11]{A.~Fuster,}
\author[29]{R.~Gaior,}
\author[7]{B.~Garc\'\i{}a,}
\author[76]{D.~Garcia-Pinto,}
\author[e]{F.~Gat\'e,}
\author[34]{H.~Gemmeke,}
\author[71]{A.~Gherghel-Lascu,}
\author[28]{P.L.~Ghia,}
\author[22]{U.~Giaccari,}
\author[44]{M.~Giammarchi,}
\author[68]{M.~Giller,}
\author[69]{D.~G\l{}as,}
\author[35]{C.~Glaser,}
\author[1]{G.~Golup,}
\author[1]{M.~G\'omez Berisso,}
\author[9,10]{P.F.~G\'omez Vitale,}
\author[8,33]{N.~Gonz\'alez,}
\author[48,47]{A.~Gorgi,}
\author[i]{P.~Gorham,}
\author[40]{A.F.~Grillo,}
\author[12]{T.D.~Grubb,}
\author[54,45]{F.~Guarino,}
\author[18]{G.P.~Guedes,}
\author[8]{M.R.~Hampel,}
\author[4]{P.~Hansen,}
\author[1]{D.~Harari,}
\author[12]{T.A.~Harrison,}
\author[h]{J.L.~Harton,}
\author[33]{A.~Haungs,}
\author[35]{T.~Hebbeker,}
\author[33]{D.~Heck,}
\author[37]{P.~Heimann,}
\author[32]{A.E.~Herve,}
\author[12]{G.C.~Hill,}
\author[f]{C.~Hojvat,}
\author[33,8]{E.~Holt,}
\author[67]{P.~Homola,}
\author[63,65]{J.R.~H\"orandel,}
\author[26]{P.~Horvath,}
\author[26]{M.~Hrabovsk\'y,}
\author[33]{T.~Huege,}
\author[8,33]{J.~Hulsman,}
\author[52,42]{A.~Insolia,}
\author[72]{P.G.~Isar,}
\author[31]{I.~Jandt,}
\author[63,65]{S.~Jansen,}
\author[80]{J.A.~Johnsen,}
\author[8]{M.~Josebachuili,}
\author[31]{A.~K\"a\"ap\"a,}
\author[32]{O.~Kambeitz,}
\author[31]{K.H.~Kampert,}
\author[32]{I.~Katkov,}
\author[33]{B.~Keilhauer,}
\author[16]{N.~Kemmerich,}
\author[17]{E.~Kemp,}
\author[35]{J.~Kemp,}
\author[83]{R.M.~Kieckhafer,}
\author[33]{H.O.~Klages,}
\author[34]{M.~Kleifges,}
\author[9]{J.~Kleinfeller,}
\author[35]{R.~Krause,}
\author[31]{N.~Krohm,}
\author[35]{D.~Kuempel,}
\author[75]{G.~Kukec Mezek,}
\author[34]{N.~Kunka,}
\author[33]{A.~Kuotb Awad,}
\author[79]{D.~LaHurd,}
\author[35]{M.~Lauscher,}
\author[68]{R.~Legumina,}
\author[20]{M.A.~Leigui de Oliveira,}
\author[29]{A.~Letessier-Selvon,}
\author[28]{I.~Lhenry-Yvon,}
\author[32]{K.~Link,}
\author[52]{D.~Lo Presti,}
\author[70]{L.~Lopes,}
\author[57]{R.~L\'opez,}
\author[78]{A.~L\'opez Casado,}
\author[28]{Q.~Luce,}
\author[8,11]{A.~Lucero,}
\author[88]{M.~Malacari,}
\author[53,44]{M.~Mallamaci,}
\author[25]{D.~Mandat,}
\author[f]{P.~Mantsch,}
\author[4]{A.G.~Mariazzi,}
\author[77]{I.C.~Mari\c{s},}
\author[50,43]{G.~Marsella,}
\author[50,43]{D.~Martello,}
\author[58]{H.~Martinez,}
\author[57]{O.~Mart\'\i{}nez Bravo,}
\author[3]{J.J.~Mas\'\i{}as Meza,}
\author[33]{H.J.~Mathes,}
\author[31]{S.~Mathys,}
\author[82]{J.~Matthews,}
\author[j]{J.A.J.~Matthews,}
\author[55,46]{G.~Matthiae,}
\author[31]{E.~Mayotte,}
\author[f]{P.O.~Mazur,}
\author[80]{C.~Medina,}
\author[62]{G.~Medina-Tanco,}
\author[8]{D.~Melo,}
\author[34]{A.~Menshikov,}
\author[80]{K.-D.~Merenda,}
\author[6]{M.I.~Micheletti,}
\author[35]{L.~Middendorf,}
\author[76]{I.A.~Minaya,}
\author[53,44]{L.~Miramonti,}
\author[71]{B.~Mitrica,}
\author[32]{D.~Mockler,}
\author[1]{S.~Mollerach,}
\author[30]{F.~Montanet,}
\author[48,47]{C.~Morello,}
\author[87]{M.~Mostaf\'a,}
\author[8,33]{A.L.~M\"uller,}
\author[35]{G.~M\"uller,}
\author[17,19]{M.A.~Muller,}
\author[33,8]{S.~M\"uller,}
\author[47]{R.~Mussa,}
\author[1]{I.~Naranjo,}
\author[62]{L.~Nellen,}
\author[12]{P.H.~Nguyen,}
\author[71]{M.~Niculescu-Oglinzanu,}
\author[37]{M.~Niechciol,}
\author[31]{L.~Niemietz,}
\author[35]{T.~Niggemann,}
\author[83]{D.~Nitz,}
\author[27]{D.~Nosek,}
\author[27]{V.~Novotny,}
\author[26]{H.~No\v{z}ka,}
\author[24]{L.A.~N\'u\~nez,}
\author[37]{L.~Ochilo,}
\author[87]{F.~Oikonomou,}
\author[88]{A.~Olinto,}
\author[25]{M.~Palatka,}
\author[2]{J.~Pallotta,}
\author[31]{P.~Papenbreer,}
\author[78]{G.~Parente,}
\author[57]{A.~Parra,}
\author[85,81]{T.~Paul,}
\author[25]{M.~Pech,}
\author[78]{F.~Pedreira,}
\author[67]{J.~P\c{e}kala,}
\author[59]{R.~Pelayo,}
\author[24]{J.~Pe\~na-Rodriguez,}
\author[17]{L.~A.~S.~Pereira,}
\author[8]{M.~Perl\'\i{}n,}
\author[50,43]{L.~Perrone,}
\author[35]{C.~Peters,}
\author[51,38,41]{S.~Petrera,}
\author[87]{J.~Phuntsok,}
\author[3]{R.~Piegaia,}
\author[33]{T.~Pierog,}
\author[3]{P.~Pieroni,}
\author[70]{M.~Pimenta,}
\author[52,42]{V.~Pirronello,}
\author[8]{M.~Platino,}
\author[35]{M.~Plum,}
\author[67]{C.~Porowski,}
\author[15]{R.R.~Prado,}
\author[88]{P.~Privitera,}
\author[25]{M.~Prouza,}
\author[2]{E.J.~Quel,}
\author[31]{S.~Querchfeld,}
\author[79]{S.~Quinn,}
\author[24]{R.~Ramos-Pollan,}
\author[31]{J.~Rautenberg,}
\author[8]{D.~Ravignani,}
\author[e]{B.~Revenu,}
\author[25]{J.~Ridky,}
\author[37]{M.~Risse,}
\author[2]{P.~Ristori,}
\author[51,41]{V.~Rizi,}
\author[16]{W.~Rodrigues de Carvalho,}
\author[55,46]{G.~Rodriguez Fernandez,}
\author[9]{J.~Rodriguez Rojo,}
\author[33]{D.~Rogozin,}
\author[8]{M.J.~Roncoroni,}
\author[33]{M.~Roth,}
\author[1]{E.~Roulet,}
\author[5]{A.C.~Rovero,}
\author[37]{P.~Ruehl,}
\author[12]{S.J.~Saffi,}
\author[71]{A.~Saftoiu,}
\author[51,41]{F.~Salamida,}
\author[57]{H.~Salazar,}
\author[75]{A.~Saleh,}
\author[87]{F.~Salesa Greus,}
\author[46]{G.~Salina,}
\author[8]{F.~S\'anchez,}
\author[77]{P.~Sanchez-Lucas,}
\author[16]{E.M.~Santos,}
\author[8]{E.~Santos,}
\author[80]{F.~Sarazin,}
\author[70]{R.~Sarmento,}
\author[8]{C.A.~Sarmiento,}
\author[9]{R.~Sato,}
\author[31]{M.~Schauer,}
\author[43]{V.~Scherini,}
\author[33]{H.~Schieler,}
\author[31]{M.~Schimp,}
\author[33,8]{D.~Schmidt,}
\author[64,c]{O.~Scholten,}
\author[25]{P.~Schov\'anek,}
\author[33]{F.G.~Schr\"oder,}
\author[32]{A.~Schulz,}
\author[35]{J.~Schumacher,}
\author[4]{S.J.~Sciutto,}
\author[39,42]{A.~Segreto,}
\author[29]{M.~Settimo,}
\author[82]{A.~Shadkam,}
\author[13]{R.C.~Shellard,}
\author[36]{G.~Sigl,}
\author[8,33]{G.~Silli,}
\author[g]{O.~Sima,}
\author[68]{A.~\'Smia\l{}kowski,}
\author[33]{R.~\v{S}m\'\i{}da,}
\author[89]{G.R.~Snow,}
\author[87]{P.~Sommers,}
\author[37]{S.~Sonntag,}
\author[12]{J.~Sorokin,}
\author[9]{R.~Squartini,}
\author[71]{D.~Stanca,}
\author[75]{S.~Stani\v{c},}
\author[67]{J.~Stasielak,}
\author[30]{P.~Stassi,}
\author[50,43]{F.~Strafella,}
\author[8,11]{F.~Suarez,}
\author[24]{M.~Suarez Dur\'an,}
\author[12]{T.~Sudholz,}
\author[28]{T.~Suomij\"arvi,}
\author[5]{A.D.~Supanitsky,}
\author[85]{J.~Swain,}
\author[69]{Z.~Szadkowski,}
\author[32]{A.~Taboada,}
\author[1]{O.A.~Taborda,}
\author[8]{A.~Tapia,}
\author[17]{V.M.~Theodoro,}
\author[65,63]{C.~Timmermans,}
\author[14]{C.J.~Todero Peixoto,}
\author[33]{L.~Tomankova,}
\author[70]{B.~Tom\'e,}
\author[78]{G.~Torralba Elipe,}
\author[25]{P.~Travnicek,}
\author[75]{M.~Trini,}
\author[33]{R.~Ulrich,}
\author[33]{M.~Unger,}
\author[35]{M.~Urban,}
\author[62]{J.F.~Vald\'es Galicia,}
\author[78]{I.~Vali\~no,}
\author[54,45]{L.~Valore,}
\author[63]{G.~van Aar,}
\author[12]{P.~van Bodegom,}
\author[64]{A.M.~van den Berg,}
\author[63]{A.~van Vliet,}
\author[57]{E.~Varela,}
\author[62]{B.~Vargas C\'ardenas,}
\author[i]{G.~Varner,}
\author[78]{R.A.~V\'azquez,}
\author[33]{D.~Veberi\v{c},}
\author[4]{I.D.~Vergara Quispe,}
\author[46]{V.~Verzi,}
\author[25]{J.~Vicha,}
\author[61]{L.~Villase\~nor,}
\author[75]{S.~Vorobiov,}
\author[4]{H.~Wahlberg,}
\author[8,11]{O.~Wainberg,}
\author[35]{D.~Walz,}
\author[a]{A.A.~Watson,}
\author[34]{M.~Weber,}
\author[33]{A.~Weindl,}
\author[80]{L.~Wiencke,}
\author[67]{H.~Wilczy\'nski,}
\author[31]{T.~Winchen,}
\author[35]{M.~Wirtz,}
\author[31]{D.~Wittkowski,}
\author[8]{B.~Wundheiler,}
\author[75]{L.~Yang,}
\author[11,8]{D.~Yelos,}
\author[8]{A.~Yushkov,}
\author[78]{E.~Zas,}
\author[75,74]{D.~Zavrtanik,}
\author[74,75]{M.~Zavrtanik,}
\author[58]{A.~Zepeda,}
\author[34]{B.~Zimmermann,}
\author[37]{M.~Ziolkowski,}
\author[28]{Z.~Zong,}
\author[52,42]{and F.~Zuccarello}

\affiliation[1]{Centro At\'omico Bariloche and Instituto Balseiro (CNEA-UNCuyo-CONICET), Argentina}
\affiliation[2]{Centro de Investigaciones en L\'aseres y Aplicaciones, CITEDEF and CONICET, Argentina}
\affiliation[3]{Departamento de F\'\i{}sica and Departamento de Ciencias de la Atm\'osfera y los Oc\'eanos, FCEyN, Universidad de Buenos Aires, Argentina}
\affiliation[4]{IFLP, Universidad Nacional de La Plata and CONICET, Argentina}
\affiliation[5]{Instituto de Astronom\'\i{}a y F\'\i{}sica del Espacio (IAFE, CONICET-UBA), Argentina}
\affiliation[6]{Instituto de F\'\i{}sica de Rosario (IFIR) -- CONICET/U.N.R.\ and Facultad de Ciencias Bioqu\'\i{}micas y Farmac\'euticas U.N.R., Argentina}
\affiliation[7]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM) and Universidad Tecnol\'ogica Nacional -- Facultad Regional Mendoza (CONICET/CNEA), Argentina}
\affiliation[8]{Instituto de Tecnolog\'\i{}as en Detecci\'on y Astropart\'\i{}culas (CNEA, CONICET, UNSAM), Centro At\'omico Constituyentes, Comisi\'on Nacional de Energ\'\i{}a At\'omica, Argentina}
\affiliation[9]{Observatorio Pierre Auger, Argentina}
\affiliation[10]{Observatorio Pierre Auger and Comisi\'on Nacional de Energ\'\i{}a At\'omica, Argentina}
\affiliation[11]{Universidad Tecnol\'ogica Nacional -- Facultad Regional Buenos Aires, Argentina}
\affiliation[12]{University of Adelaide, Australia}
\affiliation[13]{Centro Brasileiro de Pesquisas Fisicas (CBPF), Brazil}
\affiliation[14]{Universidade de S\~ao Paulo, Escola de Engenharia de Lorena, Brazil}
\affiliation[15]{Universidade de S\~ao Paulo, Inst.\ de F\'\i{}sica de S\~ao Carlos, S\~ao Carlos, Brazil}
\affiliation[16]{Universidade de S\~ao Paulo, Inst.\ de F\'\i{}sica, S\~ao Paulo, Brazil}
\affiliation[17]{Universidade Estadual de Campinas (UNICAMP), Brazil}
\affiliation[18]{Universidade Estadual de Feira de Santana (UEFS), Brazil}
\affiliation[19]{Universidade Federal de Pelotas, Brazil}
\affiliation[20]{Universidade Federal do ABC (UFABC), Brazil}
\affiliation[21]{Universidade Federal do Paran\'a, Setor Palotina, Brazil}
\affiliation[22]{Universidade Federal do Rio de Janeiro (UFRJ), Instituto de F\'\i{}sica, Brazil}
\affiliation[23]{Universidade Federal Fluminense, Brazil}
\affiliation[24]{Universidad Industrial de Santander, Colombia}
\affiliation[25]{Institute of Physics (FZU) of the Academy of Sciences of the Czech Republic, Czech Republic}
\affiliation[26]{Palacky University, RCPTM, Czech Republic}
\affiliation[27]{University Prague, Institute of Particle and Nuclear Physics, Czech Republic}
\affiliation[28]{Institut de Physique Nucl\'eaire d'Orsay (IPNO), Universit\'e Paris-Sud, Univ.\ Paris/Saclay, CNRS-IN2P3, France, France}
\affiliation[29]{Laboratoire de Physique Nucl\'eaire et de Hautes Energies (LPNHE), Universit\'es Paris 6 et Paris 7, CNRS-IN2P3, France}
\affiliation[30]{Laboratoire de Physique Subatomique et de Cosmologie (LPSC), Universit\'e Grenoble-Alpes, CNRS/IN2P3, France}
\affiliation[31]{Bergische Universit\"at Wuppertal, Department of Physics, Germany}
\affiliation[32]{Karlsruhe Institute of Technology, Institut f\"ur Experimentelle Kernphysik (IEKP), Germany}
\affiliation[33]{Karlsruhe Institute of Technology, Institut f\"ur Kernphysik (IKP), Germany}
\affiliation[34]{Karlsruhe Institute of Technology, Institut f\"ur Prozessdatenverarbeitung und Elektronik (IPE), Germany}
\affiliation[35]{RWTH Aachen University, III.\ Physikalisches Institut A, Germany}
\affiliation[36]{Universit\"at Hamburg, II.\ Institut f\"ur Theoretische Physik, Germany}
\affiliation[37]{Universit\"at Siegen, Fachbereich 7 Physik -- Experimentelle Teilchenphysik, Germany}
\affiliation[38]{Gran Sasso Science Institute (INFN), L'Aquila, Italy}
\affiliation[39]{INAF -- Istituto di Astrofisica Spaziale e Fisica Cosmica di Palermo, Italy}
\affiliation[40]{INFN Laboratori Nazionali del Gran Sasso, Italy}
\affiliation[41]{INFN, Gruppo Collegato dell'Aquila, Italy}
\affiliation[42]{INFN, Sezione di Catania, Italy}
\affiliation[43]{INFN, Sezione di Lecce, Italy}
\affiliation[44]{INFN, Sezione di Milano, Italy}
\affiliation[45]{INFN, Sezione di Napoli, Italy}
\affiliation[46]{INFN, Sezione di Roma ``Tor Vergata``, Italy}
\affiliation[47]{INFN, Sezione di Torino, Italy}
\affiliation[48]{Osservatorio Astrofisico di Torino (INAF), Torino, Italy}
\affiliation[49]{Universit\`a del Salento, Dipartimento di Ingegneria, Italy}
\affiliation[50]{Universit\`a del Salento, Dipartimento di Matematica e Fisica ``E.\ De Giorgi'', Italy}
\affiliation[51]{Universit\`a dell'Aquila, Dipartimento di Scienze Fisiche e Chimiche, Italy}
\affiliation[52]{Universit\`a di Catania, Dipartimento di Fisica e Astronomia, Italy}
\affiliation[53]{Universit\`a di Milano, Dipartimento di Fisica, Italy}
\affiliation[54]{Universit\`a di Napoli ``Federico II``, Dipartimento di Fisica ``Ettore Pancini``, Italy}
\affiliation[55]{Universit\`a di Roma ``Tor Vergata'', Dipartimento di Fisica, Italy}
\affiliation[56]{Universit\`a Torino, Dipartimento di Fisica, Italy}
\affiliation[57]{Benem\'erita Universidad Aut\'onoma de Puebla (BUAP), M\'exico}
\affiliation[58]{Centro de Investigaci\'on y de Estudios Avanzados del IPN (CINVESTAV), M\'exico}
\affiliation[59]{Unidad Profesional Interdisciplinaria en Ingenier\'\i{}a y Tecnolog\'\i{}as Avanzadas del Instituto Polit\'ecnico Nacional (UPIITA-IPN), M\'exico}
\affiliation[60]{Universidad Aut\'onoma de Chiapas, M\'exico}
\affiliation[61]{Universidad Michoacana de San Nicol\'as de Hidalgo, M\'exico}
\affiliation[62]{Universidad Nacional Aut\'onoma de M\'exico, M\'exico}
\affiliation[63]{Institute for Mathematics, Astrophysics and Particle Physics (IMAPP), Radboud Universiteit, Nijmegen, Netherlands}
\affiliation[64]{KVI -- Center for Advanced Radiation Technology, University of Groningen, Netherlands}
\affiliation[65]{Nationaal Instituut voor Kernfysica en Hoge Energie Fysica (NIKHEF), Netherlands}
\affiliation[66]{Stichting Astronomisch Onderzoek in Nederland (ASTRON), Dwingeloo, Netherlands}
\affiliation[67]{Institute of Nuclear Physics PAN, Poland}
\affiliation[68]{University of \L{}\'od\'z, Faculty of Astrophysics, Poland}
\affiliation[69]{University of \L{}\'od\'z, Faculty of High-Energy Astrophysics, Poland}
\affiliation[70]{Laborat\'orio de Instrumenta\c{c}\~ao e F\'\i{}sica Experimental de Part\'\i{}culas -- LIP and Instituto Superior T\'ecnico -- IST, Universidade de Lisboa -- UL, Portugal}
\affiliation[71]{``Horia Hulubei'' National Institute for Physics and Nuclear Engineering, Romania}
\affiliation[72]{Institute of Space Science, Romania}
\affiliation[73]{University Politehnica of Bucharest, Romania}
\affiliation[74]{Experimental Particle Physics Department, J.\ Stefan Institute, Slovenia}
\affiliation[75]{Laboratory for Astroparticle Physics, University of Nova Gorica, Slovenia}
\affiliation[76]{Universidad Complutense de Madrid, Spain}
\affiliation[77]{Universidad de Granada and C.A.F.P.E., Spain}
\affiliation[78]{Universidad de Santiago de Compostela, Spain}
\affiliation[79]{Case Western Reserve University, USA}
\affiliation[80]{Colorado School of Mines, USA}
\affiliation[81]{Department of Physics and Astronomy, Lehman College, City University of New York, USA}
\affiliation[82]{Louisiana State University, USA}
\affiliation[83]{Michigan Technological University, USA}
\affiliation[84]{New York University, USA}
\affiliation[85]{Northeastern University, USA}
\affiliation[86]{Ohio State University, USA}
\affiliation[87]{Pennsylvania State University, USA}
\affiliation[88]{University of Chicago, USA}
\affiliation[89]{University of Nebraska, USA}
\affiliation[]{-----}
\affiliation[a]{School of Physics and Astronomy, University of Leeds, Leeds, United Kingdom}
\affiliation[b]{Max-Planck-Institut f\"ur Radioastronomie, Bonn, Germany}
\affiliation[c]{also at Vrije Universiteit Brussels, Brussels, Belgium}
\affiliation[d]{now at Deutsches Elektronen-Synchrotron (DESY), Zeuthen, Germany}
\affiliation[e]{SUBATECH, \'Ecole des Mines de Nantes, CNRS-IN2P3, Universit\'e de Nantes}
\affiliation[f]{Fermi National Accelerator Laboratory, USA}
\affiliation[g]{University of Bucharest, Physics Department, Bucharest}
\affiliation[h]{Colorado State University, Fort Collins, CO}
\affiliation[i]{University of Hawaii, Honolulu, HI}
\affiliation[j]{University of New Mexico, Albuquerque, NM}

